CoMuMDR: Code-mixed Multi-modal Multi-domain corpus for Discourse paRsing in conversations

Discourse parsing is an important task useful for NLU applications such as summarization, machine comprehension, and emotion recognition. The current discourse parsing datasets based on conversations consists of written English dialogues restricted to a single domain. In this resource paper, we introduce CoMuMDR: Code-mixed Multi-modal Multi-domain corpus for Discourse paRsing in conversations. The corpus (code-mixed in Hindi and English) has both audio and transcribed text and is annotated with nine discourse relations. We experiment with various SoTA baseline models; the poor performance of SoTA models highlights the challenges of multi-domain code-mixed corpus, pointing towards the need for developing better models for such realistic settings.

==> sections/methodology.tex <==
\section{Methodology} \label{sec:methodology}
Our discourse parser consists of 3 significant components: clause identifier, link predictor, and relation classifier. The ``clause identifier'' finds a clause's first and last token and marks the tokens between them (including the start and end) as the clause span. The ``link predictor'' finds projective and forward-only links between pairs of clauses, which builds the discourse graph. The ``relation classifier'' predicts the appropriate discourse label for a link. Hence, the system divides utterances into clauses, links pairs of clauses to build a discourse graph and assigns a discourse label to each link.




==> sections/results.tex <==
% \vspace{-2mm}
% \section{Results and Analysis} \label{sec:results}
% \vspace{-2mm}

% \begin{table}[t]
% \centering
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{@{}l ccc ccc@{}}
%     \toprule
%          & \multicolumn{3}{c}{\textbf{Link only}}& \multicolumn{3}{c}{\textbf{Link + relation}} \\ 
%          & STAC & Molweni & \corpusname\ & STAC & Molweni & \corpusname\ \\ 
%          \midrule
%         \multicolumn{7}{c}{Multi-lingual embeddings} \\
%         % \midrule
%         % Deep Sequential     & 0.6941 & 0.7123 &        & \textbf{0.6318} & 0.5162 &        \\ 
%         Hierarchical        & 0.6841 & 0.7000 & 0.8036 & 0.5221 & 0.5733 & 0.4063 \\ 
%         Structure-aware     & 0.7125 & 0.8050 & 0.7782 & 0.5314 & 0.5614 & 0.4298 \\
%         SSP-BERT + SCIJE    & 0.7250 & \textbf{0.8205} & 0.7963 & \underline{0.6151} & \textbf{0.6634} & \textbf{0.6634} \\ 
%         SDDP                & 0.7304 & 0.7898 & \underline{0.8054} & 0.5670 & 0.5770 & 0.3031 \\
%         \midrule
%         \multicolumn{7}{c}{English-only embeddings} \\
%         Deep Sequential     & 0.7496 & 0.7577 & 0.7330 & \textbf{0.6318} & 0.5162 & 0.4796 \\ 
%         Hierarchical        & 0.7505 & 0.8097 & 0.8036 & 0.5704 & 0.5690 & 0.5022 \\ 
%         Structure-aware     & 0.7267 & 0.8232 & 0.7782 & 0.5582 & \underline{0.5934} & 0.4072 \\
%         SSP-BERT + SCIJE    & 0.7201 & \textbf{0.8293} & 0.7737 & 0.5623 & 0.5925 & 0.5067 \\ 
%         SDDP                & 0.7488 & \underline{0.8233} & 0.7918 & 0.5887 & 0.5770 & 0.2941 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{F1-score of various discourse parsing models.  Values in \textbf{bold} highlight the top-performing model in each method, while values in \underline{underline} highlight the next top-performing model.}% We used the text embeddings provided with each model for the English-only embeddings and \texttt{paraphrase-xlm-r-multilingual-v1} to encode the EDUs for discourse parsing.}
%     %\caption{F1-score of various discourse parsing models on the STAC and Molweni datasets on link and link+relation prediction. Values in \textbf{bold} highlight the top-performing model in each method, while values in \underline{underline} highlight the next top-performing model. We used  \texttt{paraphrase-xlm-r-multilingual-v1} to encode the EDUs for discourse parsing in all the datasets.}
%     \label{tab:baseline-performance-xlm}
%     \vspace{-6mm}
% \end{table}

% % \begin{table}[t]
% % \centering
% % \resizebox{\columnwidth}{!}{
% %     \begin{tabular}{@{}l|ccc|ccc@{}}
% %     \toprule
% %          & \multicolumn{3}{c|}{\textbf{Link only}}& \multicolumn{3}{c}{\textbf{Link + relation}} \\ 
% %          & STAC & Molweni & \corpusname\ & STAC & Molweni & \corpusname\ \\ 
% %         \midrule
% %         Deep Sequential     & 0.7496 & 0.7577 & 0.7330 & \textbf{0.6318} & 0.5162 & 0.4796 \\ 
% %         Hierarchical        & 0.7505 & 0.8097 & 0.8036 & 0.5704 & 0.5690 & 0.5022 \\ 
% %         Structure-aware     & 0.7267 & 0.8232 & 0.7782 & 0.5582 & \underline{0.5934} & 0.4072 \\
% %         SSP-BERT + SCIJE    & 0.7201 & \textbf{0.8293} & 0.7737 & 0.5623 & 0.5925 & 0.5067 \\ 
% %         SDDP                & 0.7488 & \underline{0.8233} & 0.7918 & 0.5887 & 0.5770 & 0.2941 \\ 
% %         \bottomrule
% %     \end{tabular}
% %     }
% %      \caption{F1-score of various discourse parsing models. Values in \textbf{bold} highlight the top-performing model in each method, while values in \underline{underline} highlight the next top-performing model. We used the default text encoders for EDUs in all the datasets.}
% %    % \caption{F1-score of various discourse parsing models on the STAC and Molweni datasets on link and link+relation prediction. Values in \textbf{bold} highlight the top-performing model in each method, while values in \underline{underline} highlight the next top-performing model. We used the default text encoders for EDUs in all the datasets.}
% %     \label{tab:baseline-performance-bert}
% % \end{table}

% Table \ref{tab:baseline-performance-xlm} shows the F1-score (App. \ref{app:eval-metric}) on test sets for link and link+relation prediction. %of the respective models and datasets on English-only and multilingual embeddings respectively for the tasks of link prediction and link+relation prediction. 
% For both the settings, \corpusname\ scores are lowest across all the models, highlighting the challenge of discourse parsing on multi-domain, multilingual conversations. %We also implemented the discourse parsing models with multilingual text embedding models as \corpusname\ consists of hindi-english code-mixed conversations. We used the \texttt{paraphrase-xlm-r-multilingual-v1} to encode the EDUs and pass the same through the models to obtain link prediction and relation classification. Here, 
% As can be observed, our data has an equivalent score across models for link prediction. SDDP and Hierarchical model outperform on \corpusname\ compared to STAC and Molweni. However, in relation classification (link+relation), \corpusname\ has the lowest performance possibly due to presence of multiple domains and challenge of domain adaptation \cite{liu-chen-2021-improving}. 
% %highlighting the difficulty in relation classification in a multi-domain dataset, further indicating the point about domain adaptation  \cite{liu-chen-2021-improving}.

% \noindent\textbf{Error Analysis:} On further analysis, we observed that the hierarchical model \cite{liu-chen-2021-improving} could not predict the same relation links for ``Correction'' and ``Contrast'' on \corpusname, leading to a loss of performance in link prediction and relation classification involving correction and contrast. The hierarchical model could easily identify ``Acknowledgement'' relations among the correctly predicted links. It could be due to the strong presence ($\sim 18\%$) of ``Acknowledgement'' in the dataset. Similarly, in SSP-BERT, the model misclassified some ``Acknowledgement'' relations as ``Question answer pairs''. App. Fig. \ref{fig:error-sample-1} is an example of a conversation snippet with the gold and predicted relations marked on the left and right sides, respectively. The model incorrectly classified an ``Acknowledgement'' relation as a ``Question answer pair'', possibly due to the presence of ``ma'am'' in the acknowledgment clause (also see App. Fig. \ref{fig:error-sample-1}). 
% % The SOTA and other baseline methods of discourse parsing do not perform at par with STAC or Molweni when trained and evaluated on our dataset, CoMuMDR. We find that link prediction scores are low for certain relationship types. However, we do not provide relationship-type information to the models during training or predicting the links. 
% In Table \ref{tab:baseline-performance-xlm}, we have computed the results of link and link+relation prediction of SDDP using Roberta and \texttt{paraphrase-xlm-r-multilingual-v1}. Roberta handles English-only text and cannot handle code-mixed or Hindi text. On the other hand, paraphrase-xlm-r-multilingual-v1 can handle multilingual text but often fails at effectively processing code-mixed text. Thus, Table \ref{tab:baseline-performance-xlm} shows lower performance on relation prediction for SDDP. Baseline methods, including Deep sequential, hierarchical, Structure-aware, SSP-Bert + SCIJE, perform relation prediction after link prediction, i.e., they classify the relation type for each predicted link. On the other hand, SDDP performs link+relation prediction simultaneously as a single task, which is much more complicated. Hence, SDDP shows significantly lower performance on link+relation prediction than other baseline methods. Additionally, SDDP assumes the discourse relations to form a tree and performs tree parsing during inference, while most of the discourse relations in CoMuMDR cannot adhere to tree structures. Hence, SDDP on CoMuMDR shows low scores on link+relation prediction. 

% \begin{table}[t]
% % \resizebox{\columnwidth}{!}{
%     \centering
%     \tiny
%     \begin{tabular}{l cc}
%     \toprule
%         ~ & \textbf{Link only} & \textbf{Link+relation} \\ 
%         \midrule
%         STAC & 0.6012 & \textbf{0.2729} \\
%         Molweni & 0.5176 & 0.1474 \\
%         \corpusname & \textbf{0.6852} & 0.2507 \\ 
%     \bottomrule
%     \end{tabular}
%     % }
%     \caption{Performance of GPT-4 as a discourse parser} % on STAC, Molweni and \corpusname. We prompted GPT-4 with 3-shot examples and collected the links and relations to calculate the performance on the test sets.}
%     \label{tab:llm-scores}
%     \vspace{-5mm}
% \end{table}

% \noindent\textbf{Results of GPT-4 Model:} We evaluated GPT-4o on the test set (350 dialogues, 3500 utterances)) due to costs. We prompted GPT-4 in a 3-shot setting (template in App. \ref{app:gpt-4-template}) to behave as a discourse parser (results in Table \ref{tab:llm-scores}). GPT-4 performs worse on both tasks compared to the SoTA models. On examining the confusion matrix (App. Table \ref{tab:gpt-confusion-matrix}) for GPT-4 on \corpusname, we noticed the misclassification of ``Acknowledgement'' as ``Question answer pair'', similar to prior discourse parsing models. Additionally, we observed misclassification of ``Question extension'' as ``Continuation'', possibly due to the overlapping semantics of these relations in a two-party conversation.

% %We then computed the link prediction and relation classification scores to compare LLM-based discourse parsing with available parsers on STAC, Molweni, and \corpusname. \corpusname\ performs worse than STAC and Molweni in relation classification. Upon observing the confusion matrix for GPT-4 on \corpusname, we noticed the misclassification of ``Acknowledgement'' as ``Question answer pair'', similar to prior discourse parsing models. Additionally, we observed misclassification of ``Question extension'' as ``Continuation'', possibly due to the overlapping semantics of these relations in a two-party conversation.

% %In Table \ref{tab:llm-scores} we prompted GPT-4 in a 3-shot setting to behave as a discourse parser. We then computed the link prediction and relation classification scores to compare LLM-based discourse parsing with available parsers on STAC, Molweni, and \corpusname. \corpusname\ performs worse than STAC and Molweni in relation classification. Upon observing the confusion matrix for GPT-4 on \corpusname, we noticed the misclassification of ``Acknowledgement'' as ``Question answer pair'', similar to prior discourse parsing models. Additionally, we observed misclassification of ``Question extension'' as ``Continuation'', possibly due to the overlapping semantics of these relations in a two-party conversation.

% %We experimented with multiple discourse parsing models on prior discourse parsing datasets, including STAC, Molweni, and \corpusname. We present the results of f1-scores of the various models and datasets on link prediction and link+relation prediction in Table \ref{tab:baseline-performance-bert} and Table \ref{tab:baseline-performance-xlm}. \corpusname\ scores lower across all the models, underscoring the challenge of discourse parsing on multi-domain conversations. We marked the top-performing model score on each dataset in bold and the next top-performing score with an underline.

% % In Table \ref{tab:baseline-performance-bert} we notice that \corpusname\ scores lower than STAC and Molweni for the current state-of-the-art models, in both link prediction and link and relation prediction, highlighting the challenges of discourse parsing in audio conversations. Specifically, \corpusname\ performs lower across all the baseline models, highlighting its complexity. In link prediction, SSP-BERT and SDDP show the highest performance on Molweni, while in relation classification (performed after predicting links), the Deep sequential and Structure-aware models show the highest performance on STAC and Molweni datasets, respectively. Hence, \corpusname\ provides a stronger benchmark to evaluate discourse parsing models.

% % We also implemented the discourse parsing models with multilingual text embedding models as \corpusname\ consists of hindi-english code-mixed conversations. We used the \texttt{paraphrase-xlm-r-multilingual-v1} to encode the EDUs and pass the same through the models to obtain link prediction and relation classification. Here we see that our data has an equivalent score across models for link prediction. SDDP and Hierarchical model show higher performance on \corpusname\ compared to STAC and Molweni. However, in relation classification (link+relation), \corpusname\ has the lowest performance, highlighting the difficulty in relation classification in a multi-domain dataset, further proving the point about domain adaptation in \citet{liu-chen-2021-improving}.

% % SDDP \cite{}

% % \section {Error analysis}
% % % Which types of labels

% % % which models are best

% % % relation wise f1-score and error analysis across all models and datasets

% % % Comparison with LLM based discourse parsers

% % Table \ref{tab:baseline-performance-bert} highlights that the Hierarchical model performs best in \corpusname's link prediction and relation classification (link+relation prediction) task. On the other hand, in Table \ref{tab:baseline-performance-xlm}, the Hierarchical model shows the best performance in link prediction and SSP-BERT has the best performance in relation classification on \corpusname. 

% % Upon further analysis, we observed that the hierarchical model \cite{liu-chen-2021-improving} could not predict the same relation links for ``Correction'' and ``Contrast'' on \corpusname, leading to a loss of performance in link prediction and relation classification involving correction and contrast. The heirarchical model could easily identify ``Acknowledgement'' relations among the correctly predicted links. This could be due to the strong presence of ``Acknowledgement'' in the dataset, $18\%$. Similarly, in SSP-BERT, the model misclassified some ``Acknowledgement'' relations as ``Question answer pairs''. Figure \ref{fig:error-sample-1} is an example of a conversation snippet with the gold and predicted relations marked on the left and right sides, respectively. The model incorrectly classified an ``Acknowledgement'' relation as a ``Question answer pair'', possibly due to the presence of ``ma'am'' in the acknowledgment clause.

% % \begin{figure}[t]
% %     \centering
% %     \includegraphics[width=\columnwidth]{images/error_figure.pdf}
% %     \caption{A sample conversation taken from \corpusname. Utterances from the customer are marked in purple, and those of the customer center representative are green. The gold and predicted relations are marked on the left and right sides.}
% %     \label{fig:error-sample-1}
% % \end{figure}

% % In Table \ref{tab:llm-scores} we prompted GPT-4 in a 3-shot setting to behave as a discourse parser. We then computed the link prediction and relation classification scores to compare LLM-based discourse parsing with available parsers on STAC, Molweni, and \corpusname. \corpusname\ performs worse than STAC and Molweni in relation classification. Upon observing the confusion matrix for GPT-4 on \corpusname, we noticed the misclassification of ``Acknowledgement'' as ``Question answer pair'', similar to prior discourse parsing models. Additionally, we observed misclassification of ``Question extension'' as ``Continuation'', possibly due to the overlapping semantics of these relations in a two-party conversation.

% % \begin{table}[t]
% % % \resizebox{\columnwidth}{!}{
% %     \centering
% %     \begin{tabular}{l|cc}
% %     \toprule
% %         ~ & \textbf{Link only} & \textbf{Link+relation} \\ 
% %         \midrule
% %         STAC & 0.6012 & \textbf{0.2729} \\
% %         Molweni & 0.5176 & 0.1474 \\
% %         Ours & \textbf{0.6852} & 0.2507 \\ 
% %     \bottomrule
% %     \end{tabular}
% %     % }
% %     \caption{Performance of GPT-4 as a discourse parser on STAC, Molweni and \corpusname. We prompted GPT-4 with 3-shot examples and collected the links and relations to calculate the performance on the test sets.}
% %     \label{tab:llm-scores}
% % \end{table}

